Fast-dRRT*: Efficient Multi-Robot Motion Planning for Automated Industrial Manufacturing

We present Fast-dRRT*, a sampling-based multi-robot planner, for real-time industrial automation scenarios. Fast-dRRT* builds upon the discrete rapidly-exploring random tree (dRRT*) planner, and extends dRRT* by using pre-computed swept volumes for efficient collision detection, deadlock avoidance for partial multi-robot problems, and a simplified rewiring strategy. We evaluate Fast-dRRT* on five challenging multi-robot scenarios using two to four industrial robot arms from various manufacturers. The scenarios comprise situations involving deadlocks, narrow passages, and close proximity tasks. The results are compared against dRRT*, and show Fast-dRRT* to outperform dRRT* by up to 94% in terms of finding solutions within given time limits, while only sacrificing up to 35% on initial solution cost. Furthermore, Fast-dRRT* demonstrates resilience against noise in target configurations, and is able to solve challenging welding, and pick and place tasks with reduced computational time. This makes Fast-dRRT* a promising option for real-time motion planning in industrial automation.

==> todo.tex <==
\andreas{
\begin{itemize}
    \item Introduction: Done, needs Re-read/editing
    \item Related work: Needs complete revamp to put it into max 2 pages. 
    \item Background: Could use dRRT* summary
    \item Method: Needs figures, and restructuring. Add pseudocode for each feature (alternate location, different Fast-dRRT*)
    \item Evaluation: Explain results
    \item Conclusion: Done, needs Re-read/editing
\end{itemize}
}
